Fair and Diverse Allocation of Scarce Resources

We aim to design a fairness-aware allocation approach to maximize the geographical diversity and avoid unfairness in the sense of demographic disparity. During the development of this work, the COVID-19 pandemic is still spreading in the U.S. and other parts of the world on large scale. Many poor communities and minority groups are much more vulnerable than the rest. To provide sufficient vaccine and medical resources to all residents and effectively stop the further spreading of the pandemic, the average medical resources per capita of a community should be independent of the community's demographic features but only conditional on the exposure rate to the disease. In this article, we integrate different aspects of resource allocation and seek a synergistic intervention strategy that gives vulnerable populations with higher priority when distributing medical resources. This prevention-centered strategy is a trade-off between geographical coverage and social group fairness. The proposed principle can be applied to other scarce resources and social benefits allocation.

==> background.tex <==
\section{Background}\label{sec:back}

In this section, we introduce the allocation model and the fairness notions.

\subsection{Allocation Model}
Once an outbreak is detected, public health authorities will initiate attempt to intervene further spread designing various policies and actions such as vaccines, anti-infective treatments, and social distancing.  %(Wallinga, van Boven, & Lipsitch, 2010). 
In this research, we study the optimal vaccine allocation in a region consisting of geographic and demographic subgroups in a pandemic situation. 

% Research has shown that a vaccine is perhaps the most effective way of protecting the population from an epidemic of infectious diseases (Levi, 2009).  In particular, vaccination at the early stages of the outbreak has been proved to be even more effective (Khazeni, 2009; Yarmand, 2010a).






\subsection{Fairness Notions}

We define a fairness constraint based on the notion of group fairness i.e. \emph{Equality of Opportunity}%~\cite{}

% Vaccine stockpiles are usually centralized and controlled by a national or state level
% organization. This organization then allocates vaccine doses to different regions under its
% jurisdiction. For example, during the 2009–2010 H1N1 pandemic, vaccine doses were
% delivered to state health departments, where they were distributed to county health
% departments. Under a multi-phase vaccination policy the lead organization would need to
% decide how many vaccine doses to allocate to each region in each phase. (yarmand)



Distributional equity that health-care decision-makers must consider when
introducing new interventions in resource-limited settings is critically important in terms of potential ethical considerations. There could be concerns
about race, gender, and age equity that might be relevant to decision making in distribution of scarce medical treatments.
Equity, or fairness, aims
to minimize differences in delivery of the medical treatments among population
groups, with special reference to disadvantaged or vulnerable populations.



First-come first-served might be considered inequitable for allocation since the members of populations are assumed to have equal needs, although they do not have equal access to resources. For example, rich people easily reach to clinics to receive necessary treatments. This is not the case for lower income population. In the \emph{Horizontal Equity} people with equal need should receive equal access to treatments. Although, it may be acceptable to differentiate between population groups on the basis of age, other sensitive attributes have created controversy such as gender or race.


\subsection{Motivating Example}

==> proofs.tex <==
\section{Proofs}



==> related_work.tex <==
\section{Related work}\label{sec:related}

% Resource allocation problem has a long history in economics (e.g,\cite{monopoly}), management science (e.g,\cite{managing}), emergency response (e.g,\new{\cite{emergency,zhao2019optimizing}}), and many more domains. 
% Healthcare resource allocation is one of the most challenging allocation problems. 
% A large number works have been developed to identify effective strategies for medical resource allocation \cite{becker1997optimal,tanner2008finding,yarmand2014optimal,matrajt2013optimal,feng2017multiobjective,ho2019branch,bertsimas2013fairness,emanuel2020fair}.

Resource allocation has been a classic and important problem in many domains such as economy (e.g,\cite{monopoly}), management science (e.g,\cite{managing}), emergency response (e.g,\cite{emergency,zhao2019optimizing}), etc. \new{
More recent works have addressed the need for an integrated approach with different purposes such as material allocation in a production plan \cite{Added-paper1}, supplier selection, and order allocation application\cite{Added-paper2}.}
Healthcare resource allocation is one of the most challenging allocation problems. 
A large number works have been developed to identify effective strategies for it \cite{becker1997optimal,tanner2008finding,yarmand2014optimal,matrajt2013optimal,feng2017multiobjective,ho2019branch,bertsimas2013fairness,emanuel2020fair}.


% Recently, fairness of algorithmic decision making has been the center of attention of many researchers designing and developing algorithms for different purposes, such as machine learning, ranking, and social welfare \cite{barocas2016big,fairmlbook,vzliobaite2017measuring,dubey2020representation}.
% The notion of fairness in resource allocation has been introduced in \cite{fairness_old} and later with a more precise definition in \cite{price}. 

Recently, the fairness of algorithmic decision making has been the center of attention of many researchers, who are designing and developing algorithms for different purposes, such as machine learning, ranking, and social welfare \cite{barocas2016big,fairmlbook,vzliobaite2017measuring,dubey2020representation}. 
Mitigating the bias of an outcome from a decision model, which is mainly caused by the inherent bias in the data and societal norm, will ensure that the outcome is not favorable or adversarial toward any specific subgroups \cite{vzliobaite2017measuring,fairmlbook,corbett2017algorithmic,dwork2012fairness,hardt2016equality,zehlike2017fa,yao2017beyond}. 
One of the critical problems where the fairness of the outcome matters significantly is scarce resource allocation.
The notion of fairness in resource allocation has been introduced in \cite{fairness_old} and later with a more precise definition in \cite{price}. 

Fairness was firstly adopted in bandwidth allocation problem for computer network systems \cite{chiu1989analysis,demers1989analysis,kelly1998rate,jaffe1981bottleneck,ogryczak2007multicriteria,ogryczak2005telecommunications,lan2010axiomatic,huaizhou2013fairness,bertsimas2012efficiency}. 
In these settings, the amount of resources requested can be modified by different users. 
Besides, service allocation mainly covers a group of users and is not necessarily one-to-one allocation. 
These settings differ from the resource allocation for scarce treatments which is a one-to-one allocation problem.

Now fairness has been addressed in many resource and service allocation methods \cite{verweij2009moral, matrajt2013optimal,lum2016predict, elzayn2019fair, koonin2020strategies}. \new{The importance of ethical consideration in resource allocation and principal guidelines have been discussed in \cite{yip2021healthcare}.} 
Here we highlight a few and emphasize our difference from them. 
In \cite{elzayn2019fair}, the authors formalize a general notion of fairness for allocation problems and investigate its algorithmic consequences when the decision-maker does not know the distribution of different subgroups (defined by creditworthy or criminal background) in the population. The distribution estimation is accomplished using censored feedback (individuals who received the resource, not the true number).
In our work, we estimate the distribution of different social groups from the data using Bayes rule. 
Singh \cite{singh2020fairness} considers a fair allocation of multiple resources to multiple users and have proposed a general optimization model to study the allocation. 
Our proposed method differs from \cite{singh2020fairness} on two aspects. 
First, \cite{singh2020fairness} assumes multi-resources and multi-type users, whereas we mainly focus on resource allocation problem across different regions and different population subgroups. 
Second, \cite{singh2020fairness} aims to maximize the coverage, whereas we consider a \emph{fairness-diversity} trade-off by minimizing the diversity and fairness gaps, simultaneously, across different regions. 
Donahue et al. \cite{donahue2020fairness} considers the problem of maximizing resource utilization when the demands for the resource are distributed across multiple groups and drawn from probability distributions. 
They require equal probabilities of receiving the resource across different groups to satisfy fairness and provide upper bounds on the price of fairness over different probability distributions. 
In our proposed model, we utilize a similar fairness requirement while requiring diversity (population) consideration across different regions. 
Thus, our work is an intersection between fairness and diversity. 
Furthermore, we deal with the one-to-one allocation instead of the coverage problem.  
\new{One recent works related to COVID-19 resource allocation designed a vulnerability indicator for racial subgroups that can be used as guidelines for medical resource allocation \cite{ong2021covid}. The proposed model cannot identify other vulnerable subgroups that are not geographically clustered, thus not able to form spatially concentrated communities. In our paper, we directly identify subgroups' vulnerability using exposure rates estimated from COVID-19 cases and death. We focus on the available data to estimate the necessary parameters and perform an empirical study using the proposed Algorithm \ref{alg:tune}.} 
% It has been addressed in many works on problems related to various networking systems and bandwidth allocation \cite{chiu1989analysis,demers1989analysis,kelly1998rate,jaffe1981bottleneck,ogryczak2007multicriteria,ogryczak2005telecommunications}. \new{The importance of ethical consideration in resource allocation and principal guidelines have been discussed in \cite{yip2021healthcare}.} 
% In their settings, the amount of resources requested can be modified by different users (or subroups). 
% Besides, service allocation mainly covers a group of users and is not necessarily one-to-one allocation. 
% These settings differ from our resource allocation for scarce treatments which is a one-to-one allocation.


% Singh \cite{singh2020fairness} considers a fair allocation of multiple resources to multiple users and have proposed a general optimization model to study the allocation. 
% Our proposed method differs from \cite{singh2020fairness} on two aspects. 
% First, \cite{singh2020fairness} assumes multi-resources and multi-type users, whereas we mainly focus on resource allocation problem across different regions and different population subgroups. 
% Second, the aim is to maximize the coverage, whereas we consider a \emph{fairness-diversity} trade off minimizing the diversity and fairness gaps, simultaneously, across different regions. 
% Donahue et al. \cite{donahue2020fairness} propose maximizing coverage of resource utilization when the demand are distributed across multiple groups and drawn from probability distributions. 
% % \textcolor{blue}{This sentence should be rewritten. Correct the grammar mistake, and make it shorter. Clarify the meaning.}
% They consider a fairness requirement to ensure individuals from different groups have equal probabilities of receiving the resource while maximizing utilization. They obtained theoretical upper bounds on the price of fairness for specific families of distributions that are used to model the demand.
% % \hadis{check lulu's files}
% % Their notion of fairness is based on the maximum difference in probability of receiving the resource and provide an upper bound for the price of fairness. 
% In our proposed model, we utilize a similar fairness requirement while requiring diversity (population) consideration across different regions. 
% Thus, our work is an intersection between fairness and diversity. 
% Furthermore, we deal with one-to-one allocation not coverage problem.  
% In this paper, we propose an algorithmic approach to find a feasible allocation based on the available data and the \emph{inherent gap} across different populations and regions. 
% In \cite{elzayn2019fair}, the authors formalize a general notion of fairness for allocation problems and investigate its algorithmic consequences. 
% They learn the unknown probability distributions \textcolor{blue}{distributions of what?} using censored feedback (individuals who received the resource, not the true number) while optimizing the allocation.
% We assume the frequency of candidates in each group is known based on the population data and do not aim to discover the hidden numbers. \textcolor{blue}{This sentence is not clear. What are candidates? What are hidden numbers? Remove it.}




In this paper, we consider a fair and diverse allocation of scarce resources. 
The proposed approach is different from the existing works using the maximum utilization \cite{bolton2003consumer} or maximum coverage \cite{singh2020fairness,elzayn2019fair} objective. 
The nature of the treatment allocation problem is not the same as the coverage problems, since the former is a one-to-one assignment problem, whereas in the latter the resource can cover more than one user such as police or doctor allocation\cite{elzayn2019fair,donahue2020fairness}. 
In our work we aim to study scarce divisible resource allocation considering the trade-off between geographical diversity and social fairness. 
More specifically, we do not seek to share the vaccines equally among groups of populations. 
Instead, we aim to allocate more resource to the vulnerable populations or the ones at high risk, depending on their exposure rate, in order to prevent death / spread of the disease. 
Our proposed model can be generalized to resource allocation in other scenarios such as disaster relief. 


%the fair and diverse allocation across population subgroups on the basis of overlapping demographic intersectional subgroups (e.g. \emph{<hispanic, female, low-income >}). 
%Maximizing utilization and fairness in disaster relief resource allocation is an active area of study. 
% \textcolor{blue}{There are some duplications between this Section and Section 1.1. Can we make the literature review (and it should be shrinked) as one subsection and remove some duplications? Then change Section 1.1 to Section 1.2.}

==> technical_archive.tex <==

\section{Fair and Diverse Allocation}\label{sec:technical}
Modeling is one of the most effective tools for analyzing different vaccine allocation strategies as an intervention before putting them into action.
On the other hand, developing statistical models can assist identifying the vulnerable populations and their exposure probabilities. we are interested to investigate the optimal distribution of 
vaccines. We study the zero phase of the vaccine distribution at the beginning of
the epidemic, where only a few doses of vaccine stockpiles are available and has not been distributed before. This zero phase of distribution is critically important to intervene and fight the outbreak. We also assume that the number of infected and immune individuals are negligible to affect the distribution policy. 



We consider a centralized decision maker for allocating available $b$ units of vaccines to a set of centers $j \in M$ including clinics, hospitals, and pharmacies. 
% Consider the availability of vaccines to be distributed as $b>0$ be the amount of available vaccines to be distributed.
%Let $A_{j}$ be the number of vaccines allocated to center $j$, where $A_j\cap A_{j'}=\emptyset, \forall j', j \in Q$, and $\sum_{i=1}^m A_i=N$. 
Let $x_j$ be a random variable denoting the amount of vaccines allocated to center $j$.
%Let $R$ be the set of zipcodes defining the regions to be covered for vaccination.
Let $z_{j}$ be the list of regions (zipcodes) assigned to be covered by center $j$.
We assume there is no intersection between the list of zipcodes covered by centers i.e. $z_j \cap z_{j'}=\emptyset, \forall j, j'\in Q$.  
Let $S_1,\dotsc,S_p$ be discrete-valued sensitive variables corresponds to demographic and socioeconomic attributes. Let $\mathcal{G}$ be the collection of protected group indicators $g$.
Let $I=\{S_1 \times S_2 \times . . . \times S_p\}$ be the set of intersectional subgroups $g_i$ of sensitive variables (e.g. $<low-income, black, female>$. 
Let $s_{i,j}$ be the population size of subgroup $g_i$ in $z_j$, where $i\in I, j \in M$. 
Let $V$ be a binary variable for being vaccinated $V=\{0,1\}$.
Let $e$ be the exposure infection rate denoting the risk factor.
Let $P(e|g_i), \forall i\in I$ be the exposure rate of intersectional demographic subgroup $g_i$.


% Allocating the vaccines optimally is critically important, especially at the beginning of the pandemic. There is a tradeoff between vaccinating geographical locations, \emph{diversity}, and vaccinating vulnerable population subgroups, \emph{fairness}. 
We study the problem of optimum resource allocation estimating the exposure probabilities, which depends on demographic distribution of populations in each region and the spread of the disease. We consider the intersection of different demographic attributes such as income, age, gender, and race for defining subgroups, and will ensure the fairness across the overlapping subgroups. 

The distributions of exposed population across different groups can be assumed independent, however, the model does not require the assumption of independence and is able to handle intersectional demographic groups. We will elaborate the estimation of these distribution in \S~\ref{sec:dstbn}.

Satisfying fairness on the intersections of multiple sensitive attributes, we should ensure that the allocation of vaccines for each subgroup is sufficient. 
At the other side, respecting geographical diversity, guarantees equality in geographic distribution. In this approach we do not want to share the vaccines equally among populations groups, instead we want to allocate more to high-risk vulnerable populations according to their exposure rate to prevent death/spread of the disease %(\hadis{I think if we use tested positive data instead of death this will be associated with preventing the spread}). Other fairness constraints can also be similarly included. 

More formally, we study the following problem:
Given a limited number of vaccine resource $b$ allocate a diverse and fair number of vaccines $x_j$ to each center $j$ satisfying \emph{geographical diversity}, $\mathcal{D}(x)$, and \emph{social group fairness}, $\mathcal{F}(x)$.
%\hadis{Still thinking about the objective function. }
The goal is to mitigate inequalities considering the geographical diversity and group fairness.
We now formalize the diversity and fairness notions.

\begin{definition}{\textbf{(Geographical Diversity)}}\\
    Geographical Diversity of distribution of a set of limited resource of size $b$ among a set of centers $M$ is satisfied if $\forall j \in M$, $P(V=1) \perp z_j$.
\end{definition}

Optimizing the allocation merely considering the diversity may not guarantee fairness on sensitive attributes such as \emph{race} and \emph{gender}.
For the purpose of fair allocation, we deploy an \emph{equality of opportunity} notion of fairness \cite{dwork2012fairness}.
\begin{definition}{\textbf{(Social Group Fairness)}}\\
    Fairness of a distribution of a set of limited resource of size $b$ among a set of centers $M$ is satisfied if $\forall i \in I $, $P(V=1|e, g_i) \perp g_i$.
\end{definition}
Diversity $\mathcal{D}(x)$ and fairness $\mathcal{F}(x)$ equations, are functions of allocation variable $x_j$ as we present in Equations~\ref{eq:diversity} and \ref{eq:fairness}, respectively. As we described in definition 1 and 2, an allocation is diverse if the probability of receiving vaccine does not depend on the geographical region, and an allocation is fair if it does not depend on the the population subgroup. To formulate this independence, we consider the allocation probability of each region (subgroups) compare to the average allocation probability across all regions (subgroups).

We now show how each definition can be viewed as a special case of a general set of linear constraints of the form.
\vspace{-3mm}
\begin{equation}\label{eq:diversity}
    \mathcal{D}_j(x) = \abs*{P(v=1|z_j)-P(v=1)}= \abs*{\frac{x_j}{\sum\limits_{i\in I}s_{i,j}}-\frac{\sum\limits_{j\in M} x_j}{\sum\limits_{j\in M} \sum\limits_{i\in I} s_{i,j}}}
\end{equation}
\begin{equation}\label{eq:fairness}
\begin{split}
    & \mathcal{F}_i(x) = \abs*{P(v=1|e, g_i)-P(v=1|e)}= \\
    & \abs*{\sum\limits_{j \in M}\frac{ x_j }{\sum\limits_{i\in I} s_{i,j} \times P(e|g_i)}\times\frac{s_{i,j}}{\sum\limits_{k\in M} s_{i,k}}-\sum\limits_{i \in I} \frac{\sum\limits_{j\in M}s_{i,j}}{\sum\limits_{k\in I} \sum\limits_{j\in J}s_{k,j}}\sum\limits_{j \in M}\frac{ x_j }{\sum\limits_{i\in I} s_{i,j} \times P(e|g_i)}\times\frac{s_{i,j}}{\sum\limits_{k\in M} s_{i,k}}}
    % & \abs*{\frac{\sum\limits_{j \in M}\frac{ x_j }{\sum\limits_{i\in I} s_{i,j}}\times\frac{s_{i,j}\times P(e|g_i)}{\sum\limits_{i\in I} s_{i,j}}}{\sum\limits_{j \in M}\frac{ s_{i,j}\times P(e|g_i) }{\sum\limits_{i\in I} s_{i,j}}}  - \frac{\sum\limits_{i\in I}{\sum\limits_{j \in M}\frac{ x_j }{\sum\limits_{i\in I} s_{i,j}}\times\frac{s_{i,j}\times P(e|g_i)}{\sum\limits_{i\in I} s_{i,j}} }}{\sum\limits_{i\in I}\sum\limits_{j \in M}\frac{ s_{i,j}\times P(e|g_i) }{\sum\limits_{i\in I} s_{i,j}}}}
\end{split}
\end{equation}
More particularly, $\mathcal{D}_j(x)$ refers to the absolute difference between the fraction of the population in region $j$ to be
vaccinated and the overall fraction of the population to be vaccinated. Similarly,  $\mathcal{F}_i(x)$ refers to the absolute difference between the fraction of the exposed population $i$ in region $j$ to be
vaccinated and the overall fraction of the exposed population to be vaccinated. %The first component in Equation~\ref{eq:fairness}, corresponds to the $\frac{\text{probability of an individual in group $i$ being vaccinated}}{\text{probability of group $i$ being exposed to the disease}}$.

We aim to minimize the diversity and unfairness gaps and ideally equal to zero to satisfy the independence definitions. To do so, we consider the maximum discrimination of allocation in geographical regions, $\mathcal{D}(x)=max_{j\in M}\mathcal{D}_j(x)$, and population subgroups, $\mathcal{F}=\max_{i\in I}\mathcal{F}(x)$, to be upper bounded by $\epsilon_{\mathcal{D}}$ and $\epsilon_{\mathcal{F}}$, respectively.
In particular, we want to allocate our $b$ available doses of vaccines among different population subgroups in different regions. Suppose that to maintain diversity we need to satisfy $\mathcal{D}(x) \leq \epsilon_{\mathcal{D}}$ satisfies. To maintain fairness we need to satisfy $\mathcal{F}(x)\leq \epsilon_{\mathcal{F}}$. The violation threshold parameters $\epsilon_{\mathcal{D}}, \epsilon_{\mathcal{F}} \in [0,1]$ are relatively small by which resources allocated to a particular region and particular group reach the intended target on diversity and fairness, respectively. We wish to find the vector $X\geq 0$ that satisfies these constraints considering the capacity constraint. Let us consider the feasibility problem of the following form:
% Instead of strict equality of diversity and fairness as a result of the independence of the corresponding probabilities from the geographical region and population subgroups, 
%Note that, our problem formulation is agnostic to the fairness definition and many other previously studied definitions of fairness can also be used
%as $\mathcal{F}(X)$.
%\hadis{this is group fairness explain}
%\hadis{The goal is to achieve geographical diversity and fairness!}
\vspace{-1mm}
\begin{align}
P1:\\%\label{eq:objfunc} & \max 0^T X \\
%\nonumber &\mbox{ s.t. }\\
\label{eq:const1} &\mathcal{D}(x_j)<\epsilon_d\\
\label{eq:const2} &\mathcal{F}(x_j)<\epsilon_f\\
\label{eq:const3} &\sum_{j\in M} x_j= b\\
\label{eq:boxconst} &\;x_j \geq 0, \quad\quad \forall j \in M\\
\label{eq:int} &\;x_j\in \mathbb{Z}, \quad\quad \forall j \in M
\end{align}
where Equation~\ref{eq:const3} is the capacity constraint; it assures that the total allocation does not exceed the capacity, i.e. what is available. Each constraints measures the deviation of each objective from a targeted goal $\epsilon$.
$\mathcal{D}$ refers as to the geographical diversity set of constraints and $\mathcal{F}$ refers as to fairness set of constraints.
Note that as quantitative metric, we say that allocation is considered as fair if $\mathcal{F}(x)\leq \epsilon_f$, and allocation is considered as diverse if $\mathcal{D}(x) \leq \epsilon_d$.

Depending on the constraints, the weights
and the available scarce resources, it is possible that no feasible solution exists for the optimization problem. In this case, the
decision maker will have no choice but to relax the constraints. In \S \ref{sec:exp} we will discuss the allocation under different scenario. %\hadis{did you do talk about infeasible scenario?}

%Assuming that the objective function of \hadis{this needs to be revised}$P1$ is a constant value, 
%scalarization approach

Inspired by Lagrangian logic, we combine the diversity and fairness measures with a trade-off control hyperparameter $\alpha$, and consider the following allocation optimization problem: 
\begin{align}
P2:\\
\label{eq:objfunc3} & \min_{x_j} (1-\alpha) (\mathcal{D}(x_j))+\alpha (\mathcal{F}(x_j))\\
\nonumber &\mbox{ s.t. }\\
\label{eq:const32} &\sum_{j\in M} x_j= b\\
\label{eq:boxconst3} &\;x_j \geq 0, \quad\quad \forall j \in M\\
\label{eq:int3} &\;x_j\in \mathbb{Z},\quad\quad \forall j \in M
\end{align}

where $\alpha \in [0,1]$ is the control parameter on the importance of fairness for allocation. If $\alpha >0.5$ the objective function focuses more on the fairness in the minimization and $\mathcal{F}(X)$ will be smaller more likely. Meaning that $\mathcal{F}$ deviates less from the constraint ~\ref{eq:const2}.

This problem formulation, $P2$, allows us to consider the discrimination control parameters as both \emph{soft constraint} and \emph{hard constraint}.  In Theorem~\ref{th:1}, we prove that an optimal solution for $P2$ satisfy diversity and fairness constraints in $P1$.
%Constraint~\ref{eq:const32} is called the capacity constraint; it assures that the total allocation does not exceed the capacity, i.e. what is available. 

%The left hand side of constraints~(\ref{eq:const1}) and (\ref{eq:const2}) refers to the absolute difference between a vaccination rate of each demographic group and the overall vaccination rate. Each such constraint can be equivalently
%expressed as a pair of inequality constraints of the form. Note that, our problem formulation is agnostic to the fairness definition and many other previously studied definitions of fairness can also be used
%as Constraint\ref{eq:const2}.

Theorem~\ref{th:1} shows that given the fairness and diversity constraints, if there exist a feasible solution to $P1$ then there must exist some $\alpha$ such that the feasible solution of $P1$ is an optimum solution for $P2$. 

\begin{theorem}\label{th:1}
Let $X'\neq \emptyset$ be the set of feasible solution of $P1$. Let $A(\alpha)= (1-\alpha)\mathcal{D}(x)+\alpha \mathcal{F}(X)$. Given $x^* \in X'$, $\exists \alpha^* s.t. \{\argmin_x A(\alpha^*)|\sum_{j\in M} x_j\leq b, x_j \geq 0\} =x^*$.
\end{theorem}

\begin{proof}
We first argue that $P1$ is equivalent to the following optimization model:
\begin{align}
P':\\
\label{eq:objfunc4} & \min (\mathcal{D}(x_j))\\
\nonumber &\mbox{ s.t. }\\
\label{eq:const41} &\mathcal{F}(x_j)= \epsilon\\
\label{eq:const42} &\sum_{j\in M} x_j = b\\
\label{eq:boxconst43} &\;x_j \geq 0, \quad\quad \forall j \in M\\
\label{eq:int43} &\;x_j\in \mathbb{Z},\quad\quad \forall j \in M
\end{align}

Consider $\epsilon\in [0,\epsilon_{\mathcal{F}}]$. Let $x^*$ be the optimal solution of $P3$. Hence, $\mathcal{F}(x^*)=\epsilon\leq \epsilon_{\mathcal{F}}$ satisfies the fairness constraint of $P1$. Now, if $\mathcal{D}(x^*) \geq \epsilon_{\mathcal{D}}$, we conclude that for $\epsilon$ there does not exist a feasible solution for $P1$. Otherwise, that feasible solution would minimize $P3$.



Introducing the a Lagrangian multiplier $\lambda$, we now define the dual Lagrangian transformation of $P3$ to be: 
\begin{align}
P'':\\
\label{eq:objfunc5} & \min (\mathcal{D}(x_j))+\lambda(\mathcal{F}(x_j)-\epsilon)\\
\nonumber &\mbox{ s.t. }\\
\label{eq:const52} &\sum_{j\in M} x_j= b\\
\label{eq:boxconst53} &\;x_j \geq 0, \quad\quad \forall j \in M\\
\label{eq:int43} &\;x_j\in \mathbb{Z},\quad\quad \forall j \in M
\end{align}

Now, we argue that given $x^* \in X'$ there exists an $\alpha^*$ such that $x^*$ is an optimum of $P2$. 
Let $\lambda^*$ be the multiplier when $x^*$ is an optimum of $P4$, then $\forall x''\neq x^*$:
\[
\mathcal{D}(x^*)+\lambda^*(\mathcal{F}(x^*)-\epsilon_{\mathcal{F}}) \leq \mathcal{D}(x'')+\lambda^*(\mathcal{F}(x'')-\epsilon_{\mathcal{F}})\]
\[
\implies \mathcal{D}(x^*)+\lambda^*\mathcal{F}(x^*)-\lambda^*\epsilon_{\mathcal{F}} \leq \mathcal{D}(x'')+\lambda^*\mathcal{F}(x'')-\lambda^*\epsilon_{\mathcal{F}}
\]
\[
\implies \mathcal{D}(x^*)+\lambda^*\mathcal{F}(x^*)\leq \mathcal{D}(x'')+\lambda^*\mathcal{F}(x'')
\]
Thus, $x^*$ is an optimum of $P2$ where $\lambda^*=\frac{(1-\alpha)}{\alpha}$.
\end{proof}

Now, our objective changes to finding the $\alpha$ value for which an optimum of $P2$ is a feasible solution of $P1$. To do so, a naive approach would be a brute-force search in $[0,1]$ with a small step sizes added to $\alpha$. However, this is not a practical approach since it needs to solve the optimization problem in each iteration and as the step size decreases the exhaustive search increases and the number of times that it needs to solve $P2$ increases, accordingly. Therefore, we first show the monotonicity of $\mathcal{D}(x)$ and $\mathcal{F}(x)$ in related to $\alpha$.

\begin{theorem}
Let $x_1^*$ and $x_2^*$ be optimum solutions for $P2$ given $\alpha_1$ and $\alpha_2$, respectively, where $\alpha_2 < \alpha_1$. The monotonocity of $\mathcal{D}(x)$ and $\mathcal{F}(x)$ holds if $ \mathcal{F}(x_2^*)\leq \mathcal{F}(x_1^*)$ and $\mathcal{D}(x_2^*) \geq \mathcal{F}(x_1^*).$
\end{theorem}

\begin{proof}
Let $\beta=\frac{\alpha}{(1-\alpha)}$. Given $x_1^*$ and $x_2^*$ corresponding to $\beta_1$ and $\beta_2$, where $\beta_2<\beta_1$:
\begin{equation}\label{eq:proof21}
\mathcal{D}(x_1^*)+\beta_1\mathcal{F}(x_1^*)\leq\mathcal{D}(x_2^*)+\beta_1\mathcal{F}(x_2^*)
\end{equation}
\begin{equation}\label{eq:proof22}
\mathcal{D}(x_2^*)+\beta_2\mathcal{F}(x_2^*)\leq\mathcal{D}(x_1^*)+\beta_2\mathcal{F}(x_1^*)
\end{equation}

Adding Equations \ref{eq:proof21} and \ref{eq:proof22}, we have:
\begin{equation}\label{eq:proof23}
\beta_1\mathcal{F}(x_1^*)+\beta_2\mathcal{F}(x_2^*)\leq\beta_1\mathcal{F}(x_2^*)+\beta_2\mathcal{F}(x_1^*)
\end{equation}
\[
\implies (\beta_2-\beta_1)(\mathcal{F}(x_2^*)-\mathcal{F}(x_1^*)) \leq 0
\]
which implies $\mathcal{F}(x_2^*)\leq\mathcal{F}(x_1^*)$. The monotonicity proof for $\mathcal{D}(x)$ is the same with $\beta=\frac{(1-\alpha)}{\alpha}$. If $\alpha_2 < \alpha_1$ then $\mathcal{D}(x_1^*)>\mathcal{D}(x_2^*)$.
\end{proof}

\subsection{LP-Relaxation}
% we analyze a linear programming (LP) relaxation for the constrained allocation problem above to obtain a fractional solution.
This problem is an integer programming problem with a convex and linear set of constraints. 
We transform the optimization problem into an equivalent linear programming (LP) problem relaxing the integer constrain Equation~\ref{eq:int} and adding auxiliary variables, $ A_{\mathcal{D}}, A_{\mathcal{F}}$ for $max$ component of diversity and fairness measures. The linear transformed problem is as follows: 
\begin{align}
P3:\\
\label{eq:objfunc5} & \min (1-\alpha) A_{\mathcal{D}} +\alpha A_{\mathcal{F}}\\
\nonumber &\mbox{ s.t. }\\
\label{eq:const51} &\mathcal{D}_j(x_j)< A_{\mathcal{D}}, \forall j \in M\\
\label{eq:const52} &\mathcal{D}_j(x_j)> A_{\mathcal{D}}, \forall j \in M\\
\label{eq:const53} &\mathcal{F}_i(x_j)< A_{\mathcal{F}}, \forall i \in I\\
\label{eq:const54} &\mathcal{F}_i(x_j)> A_{\mathcal{F}}, \forall i \in I\\
\label{eq:const55} &\sum_{j\in M} x_j= b\\
\label{eq:boxconst5} &\;x_j \geq 0, \quad\quad \forall j \in M\\
%\label{eq:int5} &\;x_j\in \mathbb{Z},\quad\quad \forall j \in M
\end{align}

This is a linear program, which can be exactly solved in polynomial
time. In practice, the simplex method can be used to find the
optimal solution efficiently with common optimization libraries
like IBM CPLEX and SciPy.

Solving the resulting linear program we will obtain a fractional solution. Consequently, it is required to round the fractional solution to create a feasible solution to $P1$ with integrality constraints.
Note that the rounded solution
is not necessarily feasible for the original problem $P1$. To ensure the feasibility of the rounded solution we employ a heuristic rounding approach similar to the one in \cite{tayfur2009model}. Algorithm~\ref{alg:rounding} shows the proposed modified rounding heuristic approach. The algorithm starts with rounding the LP relaxation solution to the nearest integer values. Next, if the resource constraint, Equation~\ref{eq:const55}, is not satisfied the algorithm will reduce the allocations of the top populated areas based on the total exceeded amount. If the resource constraint is under-satisfied, the algorithm will increase top exposed populated areas based on the total remaining resources. Note that for the Diverse-only and Fair-only scenarios, for both conditions the algorithm only considers population and exposed population to sort, respectively.

\begin{wrapfigure}{R}{0.45\textwidth}
    \begin{minipage}{0.45\textwidth}
      \begin{algorithm}[H]
        \caption{{\bf Rounding Heuristic}}
        \begin{algorithmic}[1]
        \label{alg:rounding}
        \small
        \STATE Find the LP relaxation solution; solve $P3$.
        \STATE Round the fractional allocations of each region ($x_j$) to the nearest integer.
        \STATE $b'=b-\sum_{j\in M}x_j$.
        \IF{$b'<0$}
            \STATE Sort allocation based on the population.
            \STATE Decrease the allocation of top $[b']$ regions by 1.
        \ELSIF{$b'> 0$}
            \STATE Sort allocation based on the exposed population.
            \STATE Increase the allocation of top $[b']$ regions by 1.
        \ENDIF
        \STATE Return $x_j, \forall j\in M$.
        \end{algorithmic}
      \end{algorithm}
    \end{minipage}
  \end{wrapfigure}
  
%\hadis{explain the heuristic rounding and cite!}

%\subsection{Iterative Sampling-based Approach}

%\subsection{Waterfilling}


\subsection{Optimal Trade-off Parameter, $\alpha$}\label{sec:tuning}

The parameter $\alpha$ in $P3$ controls the trade-off between the diversity and fairness of the allocation decision. Using the monotonicity property of $\mathcal{D}(x)$ and $\mathcal{F}(x)$ in related to $\alpha$, we now propose an efficient search algorithm based on \emph{binary search} to find a valid solution for $P1$. 
% \begin{wrapfigure}{L}{0.5\textwidth}
%     \includegraphics[width=\linewidth]{plots/monotone.png}
%     \vspace{-5mm}
%     \caption{\small Feasible region with respect to $\alpha$.}
%     \label{fig:monotone}
% \end{wrapfigure}

Using an example we show the high-level idea of the tuning algorithm under different scenarios. In Figure~\ref{fig:monotone}, the monotonically decreasing red curve corresponds to the fairness constraint and the monotonically increasing blue curve corresponds to the diversity constraint. The dashed horizontal lines corresponds to the thresholds allowed for diversity, $\epsilon_{\mathcal{D}}$ and fairness, $\mathcal{F}(x)$ constraints, respectively, in $P1$, Equation~\ref{eq:const1} and \ref{eq:const2}. For $\alpha=\alpha_1$ we can see that $\mathcal{F}(x)$ exceeds the allowed threshold of $\epsilon_F$. Using the monotonicity property we can prune the $\alpha$ values smaller than $\alpha_1$ because for any values in that range $\mathcal{F}(x)$ is infeasible. For $\alpha=\alpha_3$ the diversity constraint is not satisfied, hence, we can prune the range of $\alpha$ for the values larger than $\alpha_3$, for the same reason. For $\alpha=\alpha_2$, both $\mathcal{D}(x)$ and $\mathcal{F}(x)$ are satisfied. Looking at the color bar below the plot, the green part shows the range of $\alpha$ where the optimum solution of $P3$ is feasible for $P1$ and the red areas show the infeasible region of $\alpha$ values. Consequently, we can prune the $\alpha$ interval evaluating the violation of diversity and fairness constraint considering the optimum solution obtained from $P3$ according to a certain $\alpha$ value.    
%\begin{wrapfigure}{L}{0.5\textwidth}
\begin{figure}[b]
    \begin{minipage}{0.5\textwidth}
        \includegraphics[width=\linewidth]{plots/monotone2.png}
    \vspace{-5mm}
    \caption{\small Feasible region with respect to $\alpha$.}
    \label{fig:monotone}
    \end{minipage}
    \begin{minipage}{0.5\textwidth}
      \begin{algorithm}[H]
        \caption{{\bf Tuning $\alpha$}}
        \begin{algorithmic}[1]
        \label{alg:tune}
        \small
        \STATE $\alpha_l=0, \alpha_u=1$
            \WHILE{$|\alpha_l-\alpha_u|<\tau$}
                \STATE $\alpha_m=\frac{\alpha_u+\alpha_l}{2}$
                \STATE $x^*=\argmin P3(\alpha_m)$ 
                \IF{$\mathcal{D}(x^*)<\epsilon_{\mathcal{D}} \& \mathcal{F}(x^*)>\epsilon_{\mathcal{F}}$}
                    \STATE $\alpha_l=\frac{\alpha_l+\alpha_m}{2}$
                \ELSIF{$\mathcal{D}(x^*)>\epsilon_{\mathcal{D}} \& \mathcal{F}(x^*)<\epsilon_{\mathcal{F}}$}
                    \STATE $\alpha_u=\frac{\alpha_u+\alpha_m}{2}$
                \ELSIF{$\mathcal{D}(x^*)<\epsilon_{\mathcal{D}} \& \mathcal{F}(x^*)<\epsilon_{\mathcal{F}}$}
                \STATE {\bf return} $x^*$
                \ELSE
                    \STATE {\bf return} $x^*=\emptyset$
                \ENDIF
            \ENDWHILE
            \STATE {\bf return} $x^*$
            \end{algorithmic}
        \end{algorithm}
    \end{minipage}
\vspace{-5mm}
\end{figure}
%\end{wrapfigure}

Algorithm \ref{alg:tune} represent the proposed tuning algorithm. The algorithm prunes the $\alpha$ region considering the diversity and the fairness constraint. Note that, the pruning will be accomplished regarding the monotonicity behavior of $\mathbb{D}(x)$ and $\mathcal{F}(x)$ with respect to $\alpha$. The algorithm starts at the middle of the $\alpha$ interval, $\alpha_m$, and solves $P3$ with that. The algorithm then splits the $\alpha$ region into half to further prune the region until a narrow feasible range of $\alpha$ is obtained. In each iteration, if the diversity is not satisfied by the solution obtained from $P3$ the algorithm prunes the $\alpha$ range for values larger than $\alpha_m$. Similarly, if the fairness constraint is not satisfied for the same solution, the algorithm prunes the $\alpha$ range for smaller values than $\alpha_m$, since it is monotonically decreasing. 
In particular, if $D(x)<\epsilon_{d}$ and $F(x)> \epsilon_{f}$, we need to put more emphasis on fairness component by increasing $\alpha_{f}$, in order to decrease the fairness gap. Subsequently, we need to increase the lower bound, that is  $\alpha_{l}=\frac{\alpha_{l}+\alpha_{m}}{2}$.
If non of the constraints are satisfied with the solution obtained from $P3$ using $\alpha_m$, there does not exist a feasible solution for $P1$. Finally, when both constraints are satisfied the algorithm returns a valid solution, which is a feasible solution to $P1$.  

% \nazanin{When we solve the optimization problem using $\alpha_{m}$, this is in fact our $\alpha_{f}$ value and $\alpha_{d}=1-\alpha_{m}$}


%, it is always negative and hence, we can consider one side of the absolute value for these two constraints. More particularly, $P(v=1|z_j)\leq P(v=1)$ and $P(v=1|e, g_i)\leq P(v=1|e), \forall j \in M$, thus, $P(v=1)-P(v=1|z_j)<\alpha_d$ and $P(v=1|e)-P(v=1|e, g_i)<\alpha_f, \forall i \in I$.
% \[
% |P(v=1|z_j)-P(v=1)|<\alpha_d, \forall j \in M
% \]
% \[
% |P(v=1|e, s_i)-P(v=1|e)|<\alpha_f, \forall i \in I
% \]
% \begin{equation}\label{eq:fairness}
%     \textcolor{blue}{wrong!}P(v=1|e, g_i)-P(v=1|e)= \frac{\sum\limits_{j \in M} x_j }{\sum\limits_{j\in M} s_{i,z_j}\times P(e|g_i)}  -\frac{\sum\limits_{j\in M} x_j }{\sum\limits_{i\in I} \sum\limits_{j \in M}  s_{i,z_j}\times P(e|g_i)}
% \end{equation}


%In this work, we aim to distribute vaccine and medical treatments to hospitals considering fairness, $P(vaccinated|exposed)\perp race$, and diversity.  

% Using a standard approach for max-min problems, we introduce an auxiliary variable $y$ to rewrite the problem as maximum linear program:

% Each such constraint can be equivalently
% expressed as a pair of inequality constraints of the form. 

% \begin{align}
% \label{eq:objfunc2} & \max 0^T X\\ %\max_{x_1,\dots,x_M,y} y \\
% \nonumber &\mbox{ s.t. }\\ 
% \label{eq:const121} &P(v=1)-P(v=1|z_j)<\alpha_d,\quad\quad \forall j \in M\\
% \label{eq:const122} &P(v=1|z_j)-P(v=1)>\alpha_d,\quad\quad \forall j \in M\\
% \label{eq:const221} &P(v=1|e)-P(v=1|e, g_i)<\alpha_f, \quad \forall i \in I\\
% \label{eq:const222} &P(v=1|e, g_i)-P(v=1|e)>\alpha_f, \quad \forall i \in I\\
% \label{eq:const32} &\sum_{j\in M} x_j\leq b\\
% %\label{eq:const42} &  x_j \geq y, \quad\quad \forall j \in M\\ 
% \label{eq:boxconst2} &\;x_j \geq 0, \quad\quad \forall j \in M\\
% \label{eq:int2} &\;x_j\in \mathbb{Z},\quad\quad \forall j \in M
% \end{align}



%Notice that, this problem is convex, but not strictly convex. This means that it is not guaranteed to have a unique solution.


% Introducing a Lagrange multiplier $\lambda_i\geq0$ for each of the fairness constraints and $\gamma_j \geq0$ for each of diversity constraints, summarized as $\lambda$ and $\gamma$, in essence, the optimization problem is equivalent to:


\subsection{Estimating the Distribution of Exposed Population}\label{sec:dstbn}
To estimate the marginal distribution of the number of high-risk individuals in each demographic group, we have access to the number of tested positive (infected) cases CITE and death by COVID data. However, we only have access to the count of individuals of each group who were infected/died from COVID-19, this is namely $P(g_i|e)$. In the proposed model we need $P(e|g_i)$, which can be calculated from the Bayes formula if we assume the relationship between the individuals' distributions across different groups is independent.

For the intersectional groups, though, we do not make any assumptions on independence. Instead, we assume the individuals infected/died across intersectional groups are drawn from a multivariate
Poisson distribution CITE in order to regard the dependence between different demographic population distributions. The Poisson distribution has been widely used for modeling multivariate count-valued data. We consider each demographic group as an independent Poisson random variables and fit a Poisson regression to get the joint marginal probabilities of exposure.

\subsection{Price of Fairness}\label{sec:pof}
We now define the Price of Fairness (PoF) as the fairness gap that is obtained by the allocation solution without any fairness constraint to the allocation solution considering the fairness constraint.
As we described in \S~\ref{sec:technical}, Equation~\ref{eq:fairness}, the  fairness constraint is defined for each population subgroups. Incorporating these constraints the optimization model, $P3$, will minimize the gap between the allocation of each subgroup and average allocation across all groups. Running $P3$ with and without the fairness constraints, we will obtain different allocation solutions and consequently different fairness and diversity gaps. This will allow us to compare fair-diverse allocation performance with the Diverse-only allocation to analyze the impact of fairness constraints, namely POF. 
%\hadis{explain the maximum gaps}
The price of fairness metric assists the decision-maker about the fairness scheme to be considered, mainly, $\epsilon_{\mathcal{D}}$ and $\epsilon_{\mathcal{F}}$. Note that there is a trade-off between diversity and fairness gap in $P3$, when the allocation scheme is more focused on diversity $\alpha$ is close to $0$. Subsequently, the problem will be maximizing diversity subject to capacity constraint. Comparing the solution of such a problem with the one that has more focus on fairness, $\alpha$ close to $1$, we expect to see a larger fairness gap and smaller diversity gap. In \S \ref{sec:exp}, we will evaluate PoF of the allocation solution obtained under different scenarios.

%\hadis{fraction of exposed pop covered by diversity only divided by the fraction of exposed pop covered by proposed model}
% Having same percentage of coverage for individuals from different communities to receive vaccines and treatments. 

% \begin{enumerate}
%     \item Define the objectives of the allocation (maximum diversity of coverage?)
%     \item Identify all sources of variation, including: factors and their levels, units for allocation (hospitals?), blocking factors (states, cities,..). two or more blocking factors nested
%     \item Choose a rule for allocating supplies to units (proportional to population? distance? community coverage?) not sure about units and blocking variables I see hospitals grouped into cities or states.
%     \item Specify the measurements to be made, the allocation procedure, and the anticipated difficulties.
%     \item Run a pilot allocation design (random assignment?).
%     \item Specify the model.
%     \item Outline the analysis.
%     \item Calculate the number of supplies that need to be allocated for full coverage.
% \end{enumerate}

% We code quantitative factors equally spaced. 

% The actual allocation of supplies to demographic groups should be done at random, subject to some restrictions imposed by the proposed design.

% assigns the units within each block to the supplies in such a way that fair demographic distribution measure is satisfied.

% .

%number of available resource:O

%set of treatments: S


%set of communities: C

% Uniformity in the design space is one of the most important properties of Space-filling 

% Given my limited budget, how can I gain as much coverage/diversity as possible?

% determine the significant factors affecting the allocation of scarce medical supplies. State, City, Hospitals/clinics, Population, Race, Age, Income, female/male ratio,...

% find the conditions that gives rise to maximum and fair coverage/diversity 

% First, we need to identify existing geographical groups that needs the vaccine.

% Then, we need to identify demographic attributes of each location. 

% There is a hierarchy:
% \begin{itemize}
%     \item distribute the supply proportional to the population of each locations (blocking)
%     \item distribute the allocated supply in each location with respect to demographic attributes 
% \end{itemize}

